Private Reinforcement Learning with PAC and Regret Guarantees

Motivated by high-stakes decision-making domains like personalized medicine where user information is inherently sensitive, we design privacy preserving exploration policies for episodic reinforcement learning (RL). We first provide a meaningful privacy formulation using the notion of joint differential privacy (JDP)--a strong variant of differential privacy for settings where each user receives their own sets of output (e.g., policy recommendations). We then develop a private optimism-based learning algorithm that simultaneously achieves strong PAC and regret bounds, and enjoys a JDP guarantee. Our algorithm only pays for a moderate privacy cost on exploration: in comparison to the non-private bounds, the privacy parameter only appears in lower-order terms. Finally, we present lower bounds on sample complexity and regret for reinforcement learning subject to JDP.

==> docs/appex_upper_bound.tex <==
\section{Upper Bound}
For any fixed $s,a,h \in \states\times\actions\times[H]$
we introduce the following notation to count events
that ocurred right before episode $t$:
$\nhatt(s,a,h)$ is
the number of times state $(s,a,h)$ is visited ,
$\rhatt(s,a,h)$ is the cumulative reward sum,
and $\mhatt(s,a,s',h)$ is the transition count from state $s$ to state
$s'$ after taking action $a$.
We use the follwing shorthand notation for the confidence intervals that we'll
use.
\begin{align*}
% \phi(s,a,h) \eqdefU \phiboundWithE
&\SamplingConfSign \eqdefU \SamplingConfVal \\
&\SamplingNoiseConfSign \eqdefU \SamplingNoiseConfVal \\
&\PrivacyConfSign \eqdefU \PrivacyConfVal
\end{align*}
where $\Eeps \eqdefU \counterBound$.
We denote by $\wt(s,a,h)$ the probability that state $s,a$ is visited
on time step $h$ on episode $t$.
%%%%%%%%%%%%%%%%%%%%
%% Concentration bounds
%%%%%%%%%%%%%%%%%%%%
\subsection{Error Bounds}
%%%%%%%%%%%%
%% Lemma
%%%%%%%%%%%%%
\begin{lemma}\label{appex:lem:nfail}
The event that
there is an episode $t$ and $s,a,h\in \states\times\actions\times[H]$ such
that
\begin{align*}
\nhatt(s,a,t)
% \leq \sqrt{\frac{2\ln{\left(\nhatt(s,a,h)/\beta\right)} }{\nhatt(s,a,h)}}
< \sum_i^t \wt(s,a,h) - \ln{\frac{5SAH}{\beta}}
\end{align*}
happends with  probability at most $\beta/5$.
\end{lemma}
%
%%%%%%%%%%%%%
%% Lemma
%%%%%%%%%%%%%
\begin{lemma}\label{appex:lem:rewardfail}
Let $r(s,a,h)$ be the mean reward. Then the event that
 there is an episode $t$ and $s,a,h\in \states\times\actions\times[H]$ such
 that
\begin{align*}
\left|
\frac{\rhatt(s,a,h)}{\nhatt(s,a,t)}
-r(s,a,h)
\right|
% \leq \sqrt{\frac{2\ln{\left(\nhatt(s,a,h)/\beta\right)} }{\nhatt(s,a,h)}}
> \SamplingConfSign
\end{align*}
happends with  probability at most $\beta/5$.
\end{lemma}
%
%%%%%%%%%%%%%
%% Lemma
%%%%%%%%%%%%%
\begin{lemma}\label{appex:lem:Vfail}
Let $\tranKer(s,a,h)$ be the true transition distribution for state action pair
$s,a,h$. And let $V^*$ be the optimal value function.
We use the shorthand notation $\widehat{\tranKer}_t$ to denote the empirical
transition distribution given by
$\widehat{\tranKer}_t(s'|s,a,h)\eqdefU\frac{\mhatt(s,a,s',h)}{\nhatt(s,a,h)}$.
Then the event that
there is an episode $t$ and $s,a,h\in \states\times\actions\times[H]$ such
that
\begin{align*}
\left|
% \sum_{s'\in\states}V^*(s')\frac{\mhatt(s,a,s',h)}{\nhatt(s,a,h)} - \tranKer(s,a,h)V^*
\left(\widehat{\tranKer}_t(s,a,h) - \tranKer(s,a,h)\right)V^*
\right|
>  H \SamplingConfSign
\end{align*}
happends with  probability at most $\beta/5$.
\end{lemma}
%
\begin{lemma}
Then the event that
there is an episode $t$ and $s,a,h\in \states\times\actions\times[H]$
such that
\begin{align*}
\left|
\ntilt(s,a,h)  - \nhatt(s,a,h)
\right|
>  \Eeps
\end{align*}
happends with  probability at most $\beta/5$.
\end{lemma}


\begin{definition}
We define the fail event $F$ as the event that one of the events
defined in lemmas \ref{appex:lem:nfail}, \ref{appex:lem:rewardfail}, \ref{appex:lem:Vfail}  is realized.
After applying union bound we get that the fail event $F$
occurs with probability at most $\beta$.
\end{definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Definition: fail events
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Fail events}
\begin{definition}\label{appex:def:failevents}
\text{Let }
$$\Eeps = \counterBound$$
and define the following fail event:
$$F =
\bigcup_t \left[ F_t^N \cup F_t^R F_t^V
\cup F_t^{PR} \cup F_t^{PN} \cup F_t^{PM}
\right]$$
\noindent where
\begin{align}
F_t^N &= \bigg\{ \exists s,a,h: \nhat_t(s,a,h) <
\frac{1}{2} \sum_{i<t} w_{i,h}(s,a) \\
	&\quad\quad\quad \quad\quad-\ln\frac{SAH}{\beta'}\bigg\} \\
%%
F_t^R &= \Bigg\{
\exists s,a,t : \left| \frac{\rhat(s,a,h)}{\nhat(s,a,h)} - r(s,a,h)\right|
\geq   \\
 &\quad\quad \sqrt{\frac{\left(
		2\ln\ln(\nhat_t(s,a,h)) + \ln\frac{3SAH}{\beta'}
	\right)}{\nhat_t(s,a,h)}
	 }
\Bigg\}\\
% %%
F_t^V &= \bigg\{
\exists{s,a,h} : |(\hat{\cP}_t(s,a,h) - \cP(s,a,h))^{\top} V_{h+1}^*| \geq \\
&\quad\quad\quad H\sqrt{
\frac{\left( 2\text{llnp}( \nhat_t(s,a,h))+ \ln\frac{3SAH}{\beta'} \right)}{\nhat_t(s,a,h)}}
\bigg\}\\
% %%
% %%
F_t^{PR} &= \left\{
\exists{s,a,h} : |\rtil_t(s,a,h) - \rhat_t(s,a,h)| \geq E
\right\}\\
%%
F_t^{PN} &= \left\{
\exists{s,a,h} : |\ntil_t(s,a,h) - \nhat_t(s,a,h)| \geq E
\right\}\\
%%
F_t^{PM} &= \{
\exists{s,a,s',h} : \\
 &\quad\quad\quad|\mtil_t(s,a,s',h)
 - \mhat_t(s,a,s',h)| \geq E
\}
% \end{dmath}
\end{align}
% \end{equation*}
%
\end{definition}
%
%
%%%%%%%%%%%%%%%%%%%%%
%% Lemma: fail probability
% \begin{lemma}
% For any $\sigma'>0$, it holds that
% \begin{equation*}\begin{aligned}
% 	\pr{\bigcup_k F_k^N} \leq  \beta'\\
% 	\pr{\bigcup_k F_k^R} \leq 2\beta'\\
% 	\pr{\bigcup_k F_k^V} \leq 2\beta'\\
% \end{aligned}	\end{equation*}
% The total failure probability of the algorithm is bounded by
% $\pr{F} \leq 5\beta' = \beta$
% \end{lemma}
%



\subsection{Nice episodes}
%%%%%%%%%%%%
%% Def: nice episodes
%%%%%%%%%%%%
\begin{definition}[Definition 2 in \cite{dann2017unifying}] Let $\wth(s',a')$ be the probability of visiting state $s'$ and taking
action $a'$ during episode $t$ and time-step $h$ after following policy $\pit$. An episode $t$ is nice if and only if for all $s,s'\in \states$,
$a,a'\in\actions$ and $h\in [H]$  the following two conditions hold:
$$\wth(s,a) \leq w_{min} \quad
\vee \quad \frac{1}{4}\sum_{i<t} w_{i,h}(s,a) \geq \ln\frac{SAH}{\beta'} + \Eeps$$
\end{definition}

%%%%%%%%%%%%
%% Lemma: nice episode bound
%%%%%%%%%%%%
\begin{lemma}[]\label{lem:niceepisode}
Let $\ntil_{t}(s,a, h)$ be the value of $\ntil(s, a, h)$
after planning in episode $t$.
Then, if an episode $t$ is nice, then on $F^c$ for all $s\in\states$, $a\in\actions$ and
$h\in[H]$ the following holds:
$$\wth(s,a) \leq w_{min} \quad
\vee \quad \ntil_t(s,a,h) \geq \frac{1}{4}\sum_{i<t} w_{i,h}(s,a)$$
\end{lemma}
\begin{proof}
Since we consider the event ${F_t^N}^c$ and event ${F_t^{PN}}$,
it holds for all $s,a,h$ triples with $\wth(s,a)>w_{min}$
%
\begin{align*}
\ntil_t(s,a,h)\geq \frac{1}{2}\sum_{i<k}w_{i,h}(s,a)
-\ln\frac{SAH}{\beta'} - \Eeps \\
\geq \frac{1}{4}\sum_{i<t} w_{i,h}(s,a)
\end{align*}
\end{proof}

%%%%%%%%%%%%
%% Lemma: number of not-nice episodes
%%%%%%%%%%%%
\begin{lemma}[Lemma E.1 in \cite{dann2017unifying}]
\label{appex:lem:notnice}
On the good event $F^c$, the number of episodes that are not
nice is at most
$$\frac{120S^2AH^4}{\alpha\eps}\polylog(S,A,H, 1/\beta)$$
\end{lemma}
\begin{proof}
If an episode $t$ is not nice, then there is $s,a,h$ with
$\wth(s,a)>w_{min}$ and $\sum_{i<t}
 < \ln\left(\frac{4SAH}{\beta'}\right) + 4\Eeps$.
 With $\Eeps \coloneqq \frac{3H}{\eps} polylog(S,A,H)$
 Since the sum of this inequality increases by at least
 $w_{min} \coloneqq \frac{\alpha}{4SH^2}$ when this happens and the right hand side stays
 constant, this situation can occur at most
 \begin{align*}
 	\frac{4SAH}{w_{min}}\left(
	\ln\frac{SAH}{\beta'} + \Eeps
	\right) \\
% 	=
% 	\frac{20S^2AH^3}{\alpha}\left(
% 	\ln\left(\frac{SAH}{\beta'}\right) +
% \frac{3H}{\eps} polylog(S,A,H)	\right) \\
\leq \frac{120S^2AH^4}{\alpha\eps}
\polylog(S,A,H, 1/\beta)
 \end{align*}
\end{proof}
%%%%%%%%%%%%
%% Lemma: number of nice episodes
%%%%%%%%%%%%
\begin{lemma}[Main rate lemma. Lemma E.2 in \cite{dann2017unifying}]
\label{appex:lem:mainrate}
Let $r\geq 1$ fix and $C>0$ which can depend polynomially on que relevant quantities and $\alpha'>0$
and let $D\geq D$ which can depend poly-logarithmically on the relevant quantities. Then
$$\sum_{h}^H\sum_{s,a\in L_{t,k}}\wth(s,a)\left(
\frac{C(\llnp{n_t(s,a,h)} + D)}{n_t(s,a,h)}
\right)^{1/r}\leq \alpha'$$
on all but at most
$$\frac{8CSAH^r}{(\alpha')^r}\text{polylog}(S,A,H,(\beta')^{-1}, (\alpha')^{-1})$$
nice episodes.
\end{lemma}


%%%%%%%%%%%%
%% Lemma: Privacy sample complexity
%%%%%%%%%%%%
\begin{lemma}[Privacy rate. similar to Lemma E.2 in \cite{dann2017unifying}]
\label{appex:lem:privacyrate}
Fix $C>0$ and $\alpha'>0$.
Let $E$ be the error bound of the counting mechanisms on all episodes
such that for any $s,a,h$
%
$$|\ntil(s,a,h)-\nhat(s,a,h)| \leq E$$
then
%
$$\sum_{h}^H\sum_{s,a\in L_{t,k}}\wth(s,a)
\frac{CE}{\ntil_t(s,a,h)} \leq \alpha'$$
\
on all but at most
$$\frac{SAHCE}{\alpha'}\text{polylog}(S,A,H,(\beta')^{-1}, (\alpha')^{-1})$$
nice episodes.
\end{lemma}
%% Begin proof of privacy rate lemma
\begin{proof}
Define
$$\Delta_t  = \sum_{h}^H\sum_{s,a\in L_{t,k}}\wth(s,a)
\frac{CE_t}{\ntil_t(s,a,h)}$$
Using lemma \ref{lem:niceepisode} and the property of nice episodes and
the fact
\begin{equation} \begin{aligned}
\sum_{i<t} w_{i,h}(s,a) &\geq 4\ln \frac{SAH}{\delta'} \geq 2 \\
\end{aligned}\end{equation}
which implies
\begin{equation} \begin{aligned}
2\sum_{i<t} w_{i,h}(s,a) &\geq 2 + \sum_{i<t} w_{i,h}(s,a)\\
\implies 2\sum_{i<t} w_{i,h}(s,a) &\geq w_{t,h}(s,a)+ \sum_{i<t} w_{i,h}(s,a)\\
\implies \sum_{i<t} w_{i,h}(s,a) &\geq \frac{1}{2} \sum_{i\leq t} w_{i,h}(s,a)\\
\end{aligned}\end{equation}
we have
$$\ntil_t(s,a,h) \geq  \frac{1}{4}\sum_{i<t} w_{i,h}(s,a)
\geq \frac{1}{8} \sum_{i\leq t} w_{i,h}(s,a)$$
%
We can bound the gap as follows
\begin{equation*}
\Delta_t  \leq 8\sum_{h}^H\sum_{s,a\in L_{t,k}}\wth(s,a)
\frac{CE_t}{\sum_{i\leq t} w_{i,h}(s,a)}
\end{equation*}
%
%
	Assume that the gap on episode $t$ is $\Delta_t > \alpha'$. In this
cas there exist at least one $(s,a,h)$ with $w_{t,h}(s,a)>w_{min}$
and
\begin{equation}\begin{aligned}\label{eq:}
8SAH\frac{CE_t}{\sum_{i\leq t} w_{i,h}(s,a)} > \alpha'\\
\implies 8CSAH^2\log(1/\delta')\frac{\log(t)^{5/2}}{\sum_{i\leq t} w_{i,h}(s,a)} > \alpha'\\
\implies \frac{8CSAH^2}{\alpha'} > \frac{\sum_{i\leq t} w_{i,h}(s,a)}{\log(t)^{5/2}}
\end{aligned} \end{equation}
\end{proof}




\subsection{Optimally gap}
%
%%%%%%%%%%%%%%%%%%%%%
%% Lemma : optimism
%%%%%%%%%%%%%%%%%%%%%
This section provides the main analysis of the PAC sample complexity. We
procede by using optimism of the Q-value policy.

\begin{lemma}{$Q$-optimism}\label{appex:lem:optimism}
On the event $F^c$, the noisy Q-function $\Qtil$ is an optimistic estimator of the true
value policy $Q^*$.
That is, with high probability, for all $s,a\in\states\times\actions$, we have $\Qtil(s, a, h) \geq Q^*(s,a, h)$
\end{lemma}
%
%
First we provide a lemma and two claims that will
be used to prove lemma \ref{lem:optimism}.

%
%%%%%%%%%%%%%%%%%%%%%
%% Claim : frac bound
%%%%%%%%%%%%%%%%%%%%%
\begin{claim}\label{claim:fracbound}
Given any $\alpha>0$, let $n,E >0$.
If $n\geq \frac{(1+\alpha)E}{\alpha}$, then
$$\frac{1}{n-E} \leq \frac{1+\alpha}{n}$$
\end{claim}


\begin{claim}\label{claim:oneOverN}
For any $n>0$ and $0\leq E< n$, we have that
$$\frac{1}{n-E} \leq \frac{1}{n} + \frac{e + e^2}{n^2}$$
\end{claim}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Lemma: h step bound
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proof}{(of claim \ref{claim:oneOverN})}
Case 1: $n-1 \leq e$:
We have that $n-1 \leq e$
\begin{align*}
\frac{1}{n} + \frac{e}{n^2} + \frac{e^2}{n^2}
\geq \frac{1}{n} + \frac{n-1}{n} + \frac{(n-1)^2}{n^2} \\
= \frac{1}{n} + 1  - \frac{1}{n} + \frac{(n-1)^2}{n^2}
= 1 +  \frac{(n-1)^2}{n^2} \geq 1 = \\
 \frac{1}{\max(1,n-e)}
\end{align*}
Case 2: $n-e>1$: We have that $\left(\frac{1}{n-e}\right) < 1$
\begin{align*}
\frac{1}{n-e} &= \frac{1}{n}+ \frac{e}{n^2} + \frac{e^2}{n^3}+\ldots  \quad \quad (\text{Taylor expansion})\\
&= \frac{1}{n}+\frac{e}{n^2}+\frac{e^2}{n^2}\left(\frac{1}{n}+\frac{e}{n^2}+\frac{e^2}{n^3}+\ldots \right) \\
&= \frac{1}{n}+\frac{e}{n^2}+\frac{e^2}{n^2}\left(\frac{1}{n-e}\right) \\
&< \frac{1}{n}+\frac{e}{n^2}+\frac{e^2}{n^2} \quad\quad (\text{use } 1/(n-e) < 1 )
\end{align*}
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Q lower bound
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{claim}\label{claim:qlowerbound}
Given a target accuracy $\alpha'$.
	Let $E$ be the error bound from the $\BM{.}$ for round $t$.
	Then on the event $F^c$, for all
	$a\in\actions$, $s,s' \in \states$, $h \in [H]$, if $\ntil(s,a,h)>\frac{(1+\alpha')E}{\alpha'}$ we have
% \begin{equation}
\begin{align}
\frac{\rtil(s,a,h) + E + \sum_{s' \in \states}
\Vtil_h(s')(\mtil(s,a, s' , h) + E) }{\max(1, \ntil(s,a,h) - E)} \\
\leq \frac{\rtil(s,a,h) + \sum_{s'\in \states}\Vtil(s')\mtil(s,a,s',h)}{\ntil(s,a,h)}\\
	\quad\quad+ \frac{(1+\alpha')(E + HSE)}{\ntil(s,a,h)}
+ (H+1)\alpha'
% = \Qtil(s,a,h)
\end{align}
% \end{equation}
\end{claim}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Q-hat lemma
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}\label{appex:lem:Qhat} Let $\widehat{Q}$ be the optimistic
empirical Q-value of algorithm \ref{alg:privateplanning} before adding noise, defined by
\begin{align*}
\widehat{Q}(s,a,h) = \frac{\rhat(s,a,h) + \sum_{s'\states} \Vtil_h(s')\mhat(s,a,s', h)}{\nhat(s,a,h)} \\
+ \phibound \\
+ (H-h)\phibound
% + \phi + (H-h)\phi
\end{align*}
then on any time step for all $s,a,h \in  \states\times\actions\times [H]$,
\begin{align}
\Qtil(s,a,h) \geq \widehat{Q}(s,a,h)
\end{align}
\end{lemma}
\begin{proof}
On event $F^c$ we get from definition \ref{def:failevents} that $|\rtil(s,a,h) - \rhat(s,a,h)| \leq E$, $|\ntil(s,a,h) - \nhat(s,a,h)| \leq E$, and $|\mtil(s,a,s', h) - \mhat(s,a,s',h)| \leq E$. Therefore we can upper bound $\widehat{Q}$ by
%
\begin{align*}
	\widehat{Q}(s,a,h)\\
	\leq \frac{\rtil(s,a,h) + E + \sum_{s'\states} \Vtil_h(s')(\mhat(s,a,s', h) + E) }{\nhat(s,a,h) - E} \\
+ \phi + (H-h)\phi\
\end{align*}
where $\phi = \phiboundWithE$.
Then using claim \ref{claim:qlowerbound} with $\alpha' = \frac{\alpha}{5H(H+1)}$ we have can upper bound the
first term of the equation:
\begin{align*}
	\widehat{Q}(s,a,h)
	\leq
\frac{\rtil(s,a,h) + \sum_{s'\in \states}\Vtil(s')\mtil(s,a,s',h)}{\ntil(s,a,h)}\\
	\quad\quad+ \frac{(1+\alpha')(E + HSE)}{\ntil(s,a,h)}
+ \frac{\alpha }{5H}
+ \phi + (H-h)\phi \\
\equiv \Qtil(s,a,h)
\end{align*}
\end{proof}
%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Value function optimism
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}[Value function optimism]\label{appex:lem:Voptimism}
	Fix any episode $t$.
	On the event $F^c$,  the
	value function from algorithm \ref{alg:privateplanning} is optimismtic.
	i.e. for all $s\in\states$ and all $h\in[H]$
	$$\Vtil_h(s) \geq V^*_{h}(s)$$
\end{lemma}
\begin{proof}
The proof proceeds by induction.
Fixing any state $s\in\states$, we must show that $\Vtil_h(s)\geq V^*_h(s)$
for all $h\in[H]$. For the base case, note that $\Vtil_{H+1}(s)=V^*_h(s)=0$.
 Now assume that for any $h\leq H$, $\Vtil_{h+1}(s) \geq V_{h+1}^*(s)$.
Then we must show that $\Vtil_h(s) \geq V_h^*(s)$:


First write out the equation for $V^*_h(s)$:
\begin{align}\label{eq:vstar}
	V^*_h(s) = \max_{a} \left(
		r(s,a,h)  + P(s,a,h)V^*_{h+1}
	\right)
\end{align}
Let $a^*$ be the action corresponding to equation ($\ref{eq:vstar}$).
Next we write out the equation for $\Vtil_h(s)$
%
\begin{align*}
	\Vtil_h(s)
	&= \max_{a}
		\frac{\rtil(s,a,h)+ \sum_{s'} \Vtil_{h+1}\mtil(s,a,s',h)}{\ntil(s,a,h)} \\
		 &\quad\quad + \conftil(s,a,h)  \\
	&\geq \frac{\rtil(s,a^*,h)+ \sum_{s'} \Vtil_{h+1}\mtil(s,a^*,s',h)}{\ntil(s,a^*,h)} \\
		 &\quad\quad + \conftil(s,a^*,h) \\
	& \eqdefU	 \Qtil(s,a^*,h)
\end{align*}
%
Next we use lemma \ref{lem:optimismQhat} which says that on event $F^c$,
$\Qtil(s,a^*,h)\geq \widehat{Q}(s,a^*,h)$
to get a lower bound for $\Vtil_h$:
\begin{align*}
	\Vtil_h(s)
\geq \frac{\rhat(s,a^*,h) + \sum_{s'\states} \Vtil_h(s')\mhat(s,a^*,s', h)}{\nhat(s,a^*,h)} \\
+ (H+1)\phihatconfL{s,a^*,h}
\end{align*}
%
Letting
\begin{align*}
\frac{\sum_{s'\states} \Vtil_h(s')\mhat(s,a^*,s', h)}{\nhat(s,a^*,h)} = \widehat{P}(s,a^*,h)\Vtil_{h+1}
\end{align*}
and applying the inductive step (i.e. $\forall_s \Vtil_{h+1}(s)\geq V^*_{h+1}(s)$) we get
%
%
\begin{align*}
	&\Vtil_h(s) \geq \frac{\rhat(s,a^*,h)}{\nhat(s,a^*,h)}  +
		\widehat{P}(s,a^*,h)V^*_{h+1} + \\
 &\quad\quad (H+1)\phihatconfL{s,a^*,h}
\end{align*}
%
%
Next we use the concentration bound from definition \ref{def:failevents}
\begin{align*}
\widehat{P}(s,a^*,h)V^*_{h+1}\geq P(s,a^*,h)V^*_{h+1} - (H)\widehat{\phi}(s,a^*, h)
\end{align*}
and then we use the definition of $V^*_h(s)$
\begin{align*}
P(s,a^*,h)V^*_{h+1} = - r(s,a^*, h) +V^*_{h}(s)
\end{align*}
to get
%
\begin{align*}
	&\Vtil_h(s) \\
		&\geq \frac{\rtil(s,a^*,h)}{\ntil(s,a^*,h)}  +
		P(s,a^*,h)V^*_{h+1} + \widehat{\phi}(s,a^*, h) \\
		&= \frac{\rtil(s,a^*,h)}{\ntil(s,a^*,h)} - r(s,a^*, h)  + \widehat{\phi}(s,a^*, h) + V^*_{h}(s) \end{align*}
Next note that on event $F^c$, we have
\begin{align*}
\frac{\rtil(s,a^*,h)}{\ntil(s,a^*,h)} - r(s,a^*, h) + \widehat{\phi}(s,a^*, h)> 0
\end{align*}
Hence it follows that $\Vtil_h(s) \geq V_h^*(s)$,
completing the proof.
\end{proof}


\begin{proof}{of lemma \ref{lem:optimism}}
Let $\widehat{Q}$ be the optimistic empirical Q-value before adding noise.
On lemma \ref{lem:Qhat}, we showed that $\Qtil(s,a,h) \geq \hat{Q}(s,a,h) $  $\forall s,a,h$.

Next, it only remains to show that $\widehat{Q} \geq Q^*$.
Let the empirical mean reward be $\bar{r}(s,a,h) = \frac{\rhat(s,a,h)}{\nhat(s,a,h)}$ and let $\hat{P} \Vtil_{h+1} = \frac{\Vtil_h(s')(\mhat(s,a,s', h)}{\nhat(s,a,h)}$. No we can write $\widehat{Q}$ as
$$\widehat{Q}(s,a,h) = \bar{r}(s,a,h) + \hat{P}\Vtil_{h+1}$$
%
\noindent On the event $F^c$ we have that
$\frac{\rhat(s,a,h)}{\nhat(s,a,h)} - r(s,a,h) \leq \phi$ and
$(\widehat{P} - P )V^*_{h+1} \leq H \phi$. Furthermore, from
the value function optimism lemma (\ref{lem:Voptimism})
we have that for all $s \in \states$, and all $h\in[H]$,
$\Vtil_h(s) \geq V_h^*(s)$. Putting it all together:
%
\begin{align}
&\widehat{Q}(s,a,h) - Q^*(s,a,h)\\
& = \bar{r}(s,a,h) - r(s,a,h) + \widehat{P}\Vtil_{h+1} - P V^*_{h+1}\\
& \quad\quad+ (H-h+1)\phi \\
&\geq \bar{r}(s,a,h) - r(s,a,h) + (\widehat{P} - P )V^*_{h+1} \\
& \quad\quad+ \phi + (H-h)\phi \\
&\geq 0
\end{align}
\end{proof}


%%%%%%%%%%%%
%% Lemma: optimality gap
%%%%%%%%%%%%
\begin{lemma}
\label{appex:lem:optgap}
Let $\pit$ be the policy played by algorithm \ref{alg:prl} during
episode $t$.
Let $\wth(s,a)$ be the probability of visiting $s$ and taking action $a$
on episode $t$ and time $h\in[H]$. Then the optimality gap is bounded by
% \begin{equation*}
% V^{\pi^*}(s_0) - V^{\pit}(s_0) \leq 2H\sum_{h=1}^H \sum_{s',a'\in\states}\wth(s',a')\widetilde{\conf}(s', a', h)
% \end{equation*}
\begin{equation}\begin{aligned}
%% use equation \ref{eq:confbound}
V^\star - V^\pi_t
&\leq \sum_{h=1}^H \bE_{s_h \sim \pi_t}
\widetilde{\conf}(s_h,\pi_t(s_h)) \\
&\leq \sum_{h=1}^H
\sum_{s',a'\in\states}\wth(s',a')
\widetilde{\conf}(s_h,\pi_t(s_h)) \\
\end{aligned}\end{equation}
\end{lemma}
%
%%%%%%%%%%%%%%
%% Begin proof
%%%%%%%%%%%%%%
\begin{proof}
\noindent Let $\bE_{s_h \sim \pi_t}\rtil_h $ be the
expected reward received during time
step $h \in [H]$ given that we follow
policy $\pi_t$.
Let $s_1, \ldots, s_H$ be random variables, where each $s_h$
represents the state visited
during time-step $h$ after following policy $\pit$.
Next observe that
%
\begin{align}\label{eq:qtilinequality}
     \left| \bE_{\pi_t}\Qtil_1(s_1,\pi_t(s_1)) -
	     \bE_{\pi_t}\left( \rtil_1 +
	     \Qtil_2(s_2,\pi_t(s_2))
	     \right)
     \right| \\
		  \leq \bE_{\pi_t}\conftil(s_1,\pi_t(s_1))
\end{align}
%
\noindent Equation \ref{eq:qtilinequality} can be verified by rewriting
the two terms as:
$$\bE_{\pit} \Qtil(s_1, \pi_t(s_1))
= \bE_{\pit}\rtil_1  + \bE_{\pit} \Vtil(s_2)
+ \bE_{\pit}\conftil(s_1, a_1, 1)$$
\noindent and
$$\bE_{\pit} \Qtil_2(s_2, \pit(s_2)) = \bE_{\pit} \Vtil(s_2)$$


\noindent Then the optimality gap on episode $t$ is
\begin{equation}\label{eq:gapboundA}
\begin{aligned}
V^\star - V^\pi_t
&= V^\star - \sum_{h=1}^H \bE_{\pi_t}r_h  \\
&= \bE_{\pi_t}  Q_1^\star(s_1,\pi^
\star(s_1)) - \sum_{h=1}^H \bE_{\pi_t}r_h \\
%% optimism
& (\text{Optimism}) \\
&\leq \bE_{\pi_t} \Qtil_1(s_1,\pi^*(s_1))
- \sum_{h=1}^H \bE_{\pi_t}r_h \\
%% Greedy
& (\text{Greedy of policy } \pi_t) \\
&\leq \bE_{\pi_t} \Qtil_1(s_1,\pi_t(s_1))
- \sum_{h=1}^H \bE_{\pi_t}r_h \\
%%%
&\leq \bE_{\pi_t} \Qtil_1(s_1,\pi_t(s_1))
- \bE_{\pi_t}r_1 -  \sum_{h=2}^H \bE_{\pi_t}r_h \\
%% use equation \ref{eq:confbound}
& (\text{Equation \ref{eq:qtilinequality}}) \\
&\leq \bE_{ \pi_t} \conftil(s_1,\pi_t(s_1), 1)
	+ \bE_{\pi_t} \Qtil_2(s_2,\pi_t(s_2)) \\
	&\quad \quad - \sum_{h=2}^H \bE_{\pi_t}r_h
\end{aligned}
\end{equation}

\noindent Since $\Qtil_{H+1}(s_h, a_h) = 0$,
applying equation (\ref{eq:qtilinequality}) $H-1$ more times, we get
\begin{equation}\begin{aligned}
%% use equation \ref{eq:confbound}
(\text{equation } \ref{eq:gapboundA})
&\leq \sum_{h=1}^H \bE_{s_h \sim \pi_t} \conftil(s_h,\pi_t(s_h), h)
\end{aligned}\end{equation}
\end{proof}


\section{Other proofs}
Proof of claim \ref{claim:oneoverNbound}.
\begin{claim}\label{appex:claim:oneoverNbound}
Let $e \in \mathbb{R}$ be any positive real number.
Then for all $x \in \mathbbm{R}$ with $x\geq 2e$ it holds that
\begin{align}
\label{eq:oneoverNinequality}
\frac{1}{x - e} \leq \frac{1}{x} + \frac{2e}{x^2}
\end{align}
\end{claim}
\begin{proof}
To prove lemma \ref{claim:oneoverNbound} we will induction
on the positive real numbers following the tools from \ref{clark2012instructor}.

This case procceds by induction.
The base case $x =2e$ is easy to show.
\begin{align*}
\frac{1}{x} + \frac{2e}{x^2} =
\frac{1}{2e} + \frac{2e}{(2e)^2} =
\frac{1}{2e} + \frac{1}{2e} =
\frac{1}{e} =  \frac{1}{x-y}
\end{align*}
where the last equality follows because $x=2e$. Thus we have shown
that inequality \ref{eq:oneoverNinequality} holds when $x = 2e$.

For the inductive step we must show that for any $z\geq 2e$ if
$\frac{1}{x-e} \leq \frac{1}{x} + \frac{2e}{x^2}$
holds on all $x\in [2e, z]$
then
$\frac{1}{y-e} \leq \frac{1}{y} + \frac{2e}{y^2}$
holds on all $y\in [z, w)$ for some some $w>z$.
Secondly we must show that
for any $z> 2e$, if
$\frac{1}{x-e} \leq \frac{1}{x} + \frac{2e}{x^2}$
holds on all $x\in [2e, z)$
then
$\frac{1}{z-e} \leq \frac{1}{z} + \frac{2e}{z^2}$
holds.

We proceed by contradiction:
Let $z \geq 2e$.
For the first step let $x \in [2e, z]$ and $y\in [z, w)$ for some $w>z$.
Then assume that
$\frac{1}{x-e} \leq \frac{1}{x} + \frac{2e}{x^2}$
holds and that
$\frac{1}{y-e} > \frac{1}{y} + \frac{2e}{y^2}$.

\begin{align}
\notag
&\frac{1}{y-e} > \frac{1}{y} + \frac{2e}{y^2} \\
\notag
\Leftrightarrow & \frac{y^2}{y-e} > y + 2e
&& \text{Multiply by $y^2$}\\
\notag
\Leftrightarrow & \frac{y^2}{y-e}  + (x-y)>  x + 2e \\
\notag
\Leftrightarrow & \frac{y^2}{(y-e)x^2}  + \frac{(x-y)}{x^2}
>  \frac{1}{x} + \frac{2e}{x^2}  && \text{Divide by $x^2>0$}\\
\notag
\Leftrightarrow & \frac{y^2}{(y-e)x^2}  + \frac{(x-y)}{x^2} > \frac{1}{x-e}
&& \text{Apply inductive assumption} \\
\notag
\Leftrightarrow & y^2   > \frac{(y-e)x^2}{x-e} -(y-e)(x-y)
&& \text{Multiply by $(y-e)x^2$} \\
\notag
\Leftrightarrow & y^2   > \frac{(y-e)x^2}{x-e} + y^2 - ye - xy + xe
&& \text{Multiply by $(y-e)x^2$} \\
\notag
\Leftrightarrow & y(x+e)  > \frac{(y-e)x^2}{x-e} + xe
&& \text{Expand} \\
\notag
\Leftrightarrow & y(x+e)(x-e)  > (y-e)x^2 + xe(x-e)
&& \text{Multiply by $(x-e)$} \\
\notag
\Leftrightarrow & yx^2 -yex + yex - ye^2   > yx^2-ex^2 + ex^2 -xe^2
&& \text{Expand} \\
\notag
\Leftrightarrow & - ye^2   > -xe^2
&& \text{Simplify} \\
\label{eq:contradiction}
\Leftrightarrow & x   > y
&& \text{Divide by $e^2$}
\end{align}
Equation \ref{eq:contradiction} contradicts the assumption that
$y\geq x$. Therefore we have shown that $\frac{1}{y-e} \leq \frac{1}{y} + \frac{2e}{y^2}$ holds.

For the next step in the proof, let $x\in [2e, z)$ and assume
$\frac{1}{x-e} \leq \frac{1}{x}+ \frac{2e}{x^2}$, then we must show
that $\frac{1}{z-e} \leq \frac{1}{z}+ \frac{2e}{z^2}$. To show this we apply the
same derivation as in the previous step to arrive at the contradiction $x>z$
which completes the proof.
\end{proof}
%


==> pseudocode/PUCB_uniform.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Optimistic Planning
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{algorithm}[h]
\label{alg:privateplanning}
\begin{algorithmic}
\caption{$\mathop{PrivOP}(t, \eps, \delta, \rhat, \nhat,\mhat)$}
% \Parameter{}
\REQUIRE Private counter algorithm $\BMname$
\INPUT  Round $t$, privacy $\eps, \delta$, counter streams $\rhat, \nhat, \mhat$
% \KwIn{A dataset $D$, Queryset $\cQ$, No-regret algorithm $\mathcal{A}$, Number of rounds $T$}
\STATE $\Eeps \coloneqq \counterBound$
\STATE $\widetilde{V}_{H+1} \coloneqq 0$;
 % \quad $M\coloneqq \frac{20 H^2 E(1+SH) (1+\alpha)}{\alpha}$
 % \quad $M\coloneqq \frac{20 H^2 E(1+SH) (1+\alpha)}{\alpha}$
\FOR{$h \gets H $ {\bfseries to} $1$}
	\FORALL{$s,a \in  \states \times \actions$}
		\STATE $\rtil(s,a,h) \coloneqq \BM{\rhat(s,a,h), t}$;
		\STATE $\ntil(s,a,h) \coloneqq \BM{\nhat(s,a,h), t}$;
		\STATE $\mtil(s,a,s',h) \coloneqq \BM{\mhat(s,a,s', h), t} \forall s'\in\states$;
 		% \STATE $\mtil(s') \coloneqq \min \left\{\ntil,
					% (\mtil(s,a,s',h))\right\}, \forall s'\in\states$
		\IF{$\ntil > \Eeps$}
			% \STATE $\phi \coloneqq \sqrt{\frac{C(\llnp{\ntil} + D)}{\max(1, \ntil - E)}} $;
			% \STATE $\phi(s,a,h) \coloneqq \phiboundShortWithE$
			\STATE $\phi(s,a,h) \coloneqq \phiboundWithE$
			\STATE $\widetilde{\phi}(s,a,h) \coloneqq \phitilbound$
			\STATE $\conftil(s,a,h) = (H+1)\phi(s,a,h) + \widetilde{\phi}(a,s,h)$
			% \STATE $\conftil(s, a, h) \coloneqq
			% 	\frac{\sqrt{C(\llnp{\ntil} + D)}
			% 		+2E + 2SHE
			% 	}{\max(1, \ntil - E)}
			% 		+ \frac{\alpha}{5}$
			\STATE $\widetilde{q} \coloneqq	\frac{
			\rtil(s,a,h)
					+ \sum_{s'\in S} \Vtil_{h+1} (s') \mtil(s,a,s', h)
			}{\ntil(s,a,h)} $
			\STATE $\Qtil(s,a, h) \coloneqq
				\min\left\{
						H, \widetilde{q} +  \conftil(s, a, h)
				\right\}$
		\ELSE
			\STATE $\Qtil(s,a, h) \coloneqq H$
		\ENDIF
	\ENDFOR
	\STATE $\Vtil_h(s) \coloneqq \max_a \Qtil_h (s,a)\quad \forall s \in \states$
\ENDFOR
\OUTPUT $\Qtil$
\end{algorithmic}
\end{algorithm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% PUCB
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{algorithm}[h]
\label{alg:prl}
\begin{algorithmic}
\caption{Private Upper Confidence Bound (PUCB)}
\REQUIRE Privacy parameter $\eps, \delta$,  failure probability $\beta$
% \Parameter{}
% \STATE \algorithmicinput:
%\STATE $T \coloneqq S^2 A^2 H^5$
\STATE $\eps' \coloneqq \eps / (3H)$
% \STATE $\Count \coloneqq \BM{T, \eps'}$

\FORALL{$s,a,s'h \in \states\times\actions\times\states\times[H]$}

	\STATE Initialize empty counter streams:
	% \vspace{-3mm}
	% \STATE $\rtil(s,a,h), \ntil(s,a,h), \mtil(s,a,s',h)\coloneqq \BM{T,\eps'}$
	\STATE $\rhat(s,a,h), \nhat(s,a,h), \mhat(s,a,s',h)\coloneqq \{\}$
% \STATE $\rhat(s, a, h) \coloneqq 0$
%  \quad $\nhat(s, a, h) \coloneqq 0$
%  \quad $\mhat(s, a, s', h) \coloneqq 0$
\ENDFOR
\FOR{$t \gets 1 $ {\bfseries to} $T$}
	% \STATE {Private planning: }$\Qtil \coloneqq \mathop{{PrivOP}}(\rtil, \ntil, \mtil, \eps)$
	\STATE {Private planning: }$\Qtil \coloneqq \mathop{{PrivOP}}(t, \eps, \delta, \rhat, \nhat, \mhat)$
	\FOR{$h \coloneqq 1$ \text{\bfseries to} $H$}
	\STATE Let $s_h$ be the state during step $h$ and episode $t$
	\STATE $a_h \coloneqq \argmax_{a'} \Qtil(s_h,a',h)$;
	\STATE $r_h \sim  \reDist(s_h, a_h, h); \quad s_{h+1}
	\sim  \tranKer(.|s_h,a_h, h);$
	\STATE Feed $1$ to counters $\rhat(s_h,a_h,h), \nhat(s_h,a_h,h)$,
	\STATE \quad\quad\quad and $\mhat(s_h,a_h,s_{h+1},h)$
	\ENDFOR
	\STATE Feed $0$ to unvisited counters.
\ENDFOR
\end{algorithmic}
\end{algorithm}


==> pseudocode/counter.tex <==
\begin{algorithm}[h]
\label{alg:infrequentMech}
\begin{algorithmic}
\caption{Infrequent Private Counter}
% \Parameter{}
\INPUT Stream $\sigma$, episode $T$, privacy parameter $\eps$
\STATE $s \coloneqq 0$
\quad $a \coloneqq 0$
\quad $i \coloneqq 1$
\WHILE{$t \leq T$}
\STATE $a \coloneqq a + \sigma(t)$
\IF{$t = i^2$}
  \STATE $i \coloneqq i + 1$
  \STATE $s \coloneqq s + a + Lap(1/\eps)$
  \STATE $a \coloneqq 0$
\ENDIF
% \STATE Output $s$ on round $t$
\ENDWHILE
\OUTPUT $s$ on round $T$
\end{algorithmic}
\end{algorithm}


==> pseudocode/square_update_counter.tex <==
\begin{algorithm}[h]
\label{alg:squareUpdateMech}
\begin{algorithmic}
\caption{Square Frequency Mechanism}
% \Parameter{}
\INPUT Stream $\sigma$, episode $T$, privacy parameter $\eps$
\STATE Initialize $S \coloneqq 0$
, $k \coloneqq 1$
, $B \coloneqq 0$
, $A \coloneqq 0$
\FOR{$t \leftarrow 1 \text{ to } T$}
\STATE $A \coloneqq A + \sigma(t)$
\STATE $B \coloneqq B + \sigma(t) + Lap(1/\eps)$
\IF{$B \geq k^2$}
  \STATE $S \coloneqq S + A + Lap(1/\eps)$
  \STATE $k \coloneqq k + 1$
  \STATE $A \coloneqq 0$
\ENDIF
% \STATE Output $s$ on round $t$
\ENDFOR
\OUTPUT $S$ on round $T$
\end{algorithmic}
\end{algorithm}

